On Neural Network Equivalence Checking using SMT Solvers

Two pretrained neural networks are deemed equivalent if they yield similar outputs for the same inputs. Equivalence checking of neural networks is of great importance, due to its utility in replacing learning-enabled components with equivalent ones, when there is need to fulfill additional requirements or to address security threats, as is the case for example when using knowledge distillation, adversarial training etc. SMT solvers can potentially provide solutions to the problem of neural network equivalence checking that will be sound and complete, but as it is expected any such solution is associated with significant limitations with respect to the size of neural networks to be checked. This work presents a first SMT-based encoding of the equivalence checking problem, explores its utility and limitations and proposes avenues for future research and improvements towards more scalable and practically applicable solutions. We present experimental results that shed light to the aforementioned issues, for diverse types of neural network models (classifiers and regression networks) and equivalence criteria, towards a general and application-independent equivalence checking approach.

==> sections/NN1.tex <==
\newcommand{\logiclabel}[1]{\,{$\scriptstyle#1$}\,}
		\newcommand{\linklabelsU}[4]{\logiclabel{+1}}
				\newcommand{\linklabelsB}[4]{\logiclabel{-1}}
				\newcommand{\linklabelsC}[4]{\logiclabel{2}}

		\newcommand{\linklabelsA}[4]{\ifnum0=#2 \logiclabel{+3} \else \logiclabel{-2} \fi}
		\begin{figure}[h]
		\begin{center}
 \begin{neuralnetwork}[height=2, layertitleheight=1cm, nodespacing=2cm, layerspacing=1.7cm]
%[height=4]
 
        \newcommand{\x}[2]{$x_#2$}
        \newcommand{\y}[2]{$y^{(2)}_#2$}
        \newcommand{\hfirst}[2]{\small $h^{(1)}_#2$}
        \newcommand{\hsecond}[2]{\small $h^{(2)}_#2$}
        \inputlayer[count=2, bias=false, title={\bf Input\\layer}, text=\x]
                   %\foreach \name / \zz in {1,...,2}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
       % \node[input neuron, pin=left:Input \#\zz] (I-\name) at (0,-\zz) {};
               

        \hiddenlayer[count=2, bias=false, title={\bf Hidden\\layer 1}, text=\hfirst] \linklayers
     \link[from layer=0, to layer=1, from node=1, to node=2,label=\linklabelsU]]
      \link[from layer=0, to layer=1, from node=1, to node=1,label=\linklabelsA]]
      \link[from layer=0, to layer=1, from node=2, to node=2,label=\linklabelsC]]
      %\link[from layer=0, to layer=1, from node=2, to node=1,label=\linklabelsU]]
        %\hiddenlayer[count=3, bias=false, title=Hidden\\layer 2, text=\hsecond] \linklayers
        \outputlayer[count=2, title={\bf Output\\layer}, text=\y] \linklayers
      \link[from layer=1, to layer=2, from node=1, to node=2,label=\linklabelsB]]
         % \link[from layer=1, to layer=2, from node=1, to node=1,label=\linklabelsU]]
          \link[from layer=1, to layer=2, from node=1, to node=1,label=\linklabelsC]]
           \link[from layer=1, to layer=2, from node=2, to node=2,label=\linklabelsA]]
    \end{neuralnetwork}
    \end{center}
    \caption{An example of a feedforward neural network with an input layer of 2 inputs ($x_1$, $x_2$), an output layer with 2 outputs ($y_1$, $y_2$) and no activation function, and 1 hidden layer with 2 neurons and a ReLU activation function.
\red{Stavros: i don't like this figure. we said we would improve it. also the ReLUs are not shown in the figure.}	
	The  values on the transitions correspond to the \emph{weights} and  the upperscript values to the biases.}
    \label{fig:NN1}
    \end{figure}

==> sections/NN1_v2.tex <==
\newcommand{\logiclabel}[1]{\,{$\scriptstyle#1$}\,}
		\newcommand{\linklabelsU}[4]{\logiclabel{+1}}
				\newcommand{\linkRelu}[4]{\logiclabel{ReLU}}
				\newcommand{\linkLinear}[4]{\logiclabel{Linear}}
				\newcommand{\linklabelsB}[4]{\logiclabel{-1}}
				\newcommand{\linklabelsC}[4]{\logiclabel{2}}

		\newcommand{\linklabelsA}[4]{\ifnum0=#2 \logiclabel{+3} \else \logiclabel{-2} \fi}
		\begin{figure}[ht!]
		\begin{center}
 \begin{neuralnetwork}[height=2, layertitleheight=1cm, nodespacing=2cm, layerspacing=1.7cm]
%[height=4]
 
        \newcommand{\x}[2]{$x_#2^{}$}
        \newcommand{\z}[2]{$z'^{(2)}_#2$}
        \newcommand{\yy}[2]{$y^{(2)}_#2$}

        \newcommand{\second}[2]{ $h_#2$}
        \newcommand{\first}[2]{ $z^{(1)}_#2$}
        \inputlayer[count=2, bias=false, title={\bf Input\\layer}, text=\x]
        \hiddenlayer[count=2, bias=false, title={\bf Hidden\\layer 1}, text=\first] \linklayers
     \link[from layer=0, to layer=1, from node=1, to node=2,label=\linklabelsU]]
      \link[from layer=0, to layer=1, from node=1, to node=1,label=\linklabelsA]]
      \link[from layer=0, to layer=1, from node=2, to node=2,label=\linklabelsC]]
      %\link[from layer=0, to layer=1, from node=2, to node=1,label=\linklabelsU]]
        \hiddenlayer[count=2, bias=false, text=\second] %\linklayers
        \link[from layer=1, to layer=2, from node=1, to node=1,label=\linkRelu]]
        \link[from layer=1, to layer=2, from node=2, to node=2,label=\linkRelu]]
        \outputlayer[count=2, title={\bf Output\\layer}, text=\yy] \linklayers
      \link[from layer=2, to layer=3, from node=1, to node=2,label=\linklabelsB]]
          
          \link[from layer=2, to layer=3, from node=1, to node=1,label=\linklabelsC]]
           \link[from layer=2, to layer=3, from node=2, to node=2,label=\linklabelsA]]
 %       \outputlayer[count=2,text=\yy] 
%\link[from layer=3, to layer=4, from node=2, to node=2,label=\linkLinear]]
%\link[from layer=3, to layer=4, from node=1, to node=1,label=\linkLinear]]

    \end{neuralnetwork}
    \end{center}
     \caption{Feedforward neural network with an input layer of 2 inputs ($x_1$, $x_2$), an output layer with 2 outputs ($y_1$, $y_2$) and no activation function, and 1 hidden layer with 2 neurons and a ReLU activation function. 
	The  values on the transitions correspond to the \emph{weights} and  the upperscript values to the biases.
	\red{improve this figure too}
    \label{fig:NN11}}
    \end{figure}

==> sections/NN2.tex <==
\renewcommand{\logiclabel}[1]{\,{$\scriptstyle#1$}\,}
		\renewcommand{\linklabelsU}[4]{\logiclabel{+1}}
				\newcommand{\linkRelu}[4]{\logiclabel{ReLU}}
				\newcommand{\linkLinear}[4]{\logiclabel{Linear}}
				\renewcommand{\linklabelsB}[4]{\logiclabel{-1}}
				\renewcommand{\linklabelsC}[4]{\logiclabel{2}}

		\renewcommand{\linklabelsA}[4]{\ifnum0=#2 \logiclabel{+3} \else \logiclabel{-2} \fi}
		\begin{figure}[ht!]
		\begin{center}
 \begin{neuralnetwork}[height=2, layertitleheight=1cm, nodespacing=2cm, layerspacing=1.7cm]
%[height=4]
 
        \newcommand{\x}[2]{$x_#2$}
        \newcommand{\z}[2]{$z'^{(2)}_#2$}
        \newcommand{\yy}[2]{$y^{}_#2$}

        \newcommand{\second}[2]{\small $h_#2$}
        \newcommand{\first}[2]{\small $z^{(1)}_#2$}
        \inputlayer[count=2, bias=false, title={\bf Input\\layer}, text=\x]
        \hiddenlayer[count=2, bias=false, title={\bf Hidden\\layer 1}, text=\first] \linklayers
     \link[from layer=0, to layer=1, from node=1, to node=2,label=\linklabelsU]]
      \link[from layer=0, to layer=1, from node=1, to node=1,label=\linklabelsA]]
      \link[from layer=0, to layer=1, from node=2, to node=2,label=\linklabelsC]]
      %\link[from layer=0, to layer=1, from node=2, to node=1,label=\linklabelsU]]
        \hiddenlayer[count=2, bias=false, text=\second] %\linklayers
        \link[from layer=1, to layer=2, from node=1, to node=1,label=\linkRelu]]
        \link[from layer=1, to layer=2, from node=2, to node=2,label=\linkRelu]]
        \outputlayer[count=2, title={\bf Output\\layer}, text=\z] \linklayers
      \link[from layer=2, to layer=3, from node=1, to node=2,label=\linklabelsB]]
          
          \link[from layer=2, to layer=3, from node=1, to node=1,label=\linklabelsC]]
           \link[from layer=2, to layer=3, from node=2, to node=2,label=\linklabelsA]]
        \outputlayer[count=2,text=\yy] 
\link[from layer=3, to layer=4, from node=2, to node=2,label=\linkLinear]]
\link[from layer=3, to layer=4, from node=1, to node=1,label=\linkLinear]]

    \end{neuralnetwork}
    \end{center}
     \caption{Reconstructed feedforward neural network with an input layer of 2 inputs ($x_1$, $x_2$), an output layer with 2 outputs ($y_1$, $y_2$) and no activation function, and 1 hidden layer with 2 neurons and a ReLU activation function. 
	The  values on the transitions correspond to the \emph{weights} and  the upperscript values to the biases.
	\red{improve this figure too}
    \label{fig:NN2}}
    \end{figure}

==> sections/NN_manual.tex <==
\begin{figure}[ht!]
    
% Input layer neurons'number
\newcommand{\inputnum}{2} 
 
% Hidden layer neurons'number
\newcommand{\hiddennum}{2}  

% Output layer neurons'number
\newcommand{\outputnum}{2} 

\begin{center}

\begin{tikzpicture}
 
% Input Layer

    \node[circle,
     %node[align=center] 
     %text centered,
 label={[align=left]\normalsize \bf Input\\ \normalsize \textbf{Layer}\\~}, 
     %label=above:{\normalsize \bf Input Layer},
        %minimum size = 7mm,
        text width=4mm,
        text height=3mm,
        fill=orange!30] (Input-1) at (0,-1*1.7) {\textcolor{orange!30}{$z_2^{[1]}$}};

    \node[circle, 
        %minimum size = 7mm,
        text width=4mm,text height=3mm,
        fill=orange!30] (Input-2) at (0,-2*1.7) {\textcolor{orange!30}{$z_2^{[1]}$}};

% Hidden Layer

    \node[circle, 
        label={[align=left]\normalsize \bf Hidden\\ \normalsize \textbf{Layer}\\~}, 
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-1) at (2,-1*1.7) {$z_1^{[1]}$};
 \node[circle, 
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-2) at (2,-2*1.7) {$z_2^{[1]}$};
 
 \foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        %minimum size = 9mm,
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden_Relu-\i) at (4,-\i*1.7) {$h_{\i}^{\textcolor{blue!50}{[1]}}$};
}
% Output Layer
  

\node[circle, 
    label={[align=left]\normalsize \bf Output\\ \normalsize \textbf{Layer}\\~}, 
        %minimum size = 8mm,
    text width=4mm,text height=3mm,
    fill=purple!50,
    yshift=(\outputnum-\inputnum)*5 mm] (Output-1) at (6,-1*1.7) %{$\textcolor{purple!20}{h_1}^{[1]}$};
    {$y_1^{[1]}$};
    
    \node[circle, 
        %minimum size = 8mm,
        text width=4mm,text height=3mm,
        fill=purple!50,
        yshift=(\outputnum-\inputnum)*5 mm
    ] (Output-2) at (6,-2*1.7){$y_2^{[1]}$};

 
% Connect neurons In-Hidden
\begin{comment}
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Input-\i) -- (Hidden-\j);   
    }
}
\end{comment}
 \draw[->, shorten >=1pt] (Input-1) -- node[above] {$-2$}(Hidden-1);
 \draw[->, shorten >=1pt] (Input-2) --  node[below]{$2$}(Hidden-2);
 \draw[->, shorten >=1pt] (Input-1) --  node[above]{$1$}(Hidden-2);
  \draw[->, shorten >=1pt] (Input-2) --  node[below]{$1$}(Hidden-1);

% Connect neurons Hidden-Out
\foreach \i in {1,...,\hiddennum}
{
    %\foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt]  (Hidden-\i) -- node[above,sloped] {\em \small ReLU}(Hidden_Relu-\i);
    }
}
 

% Connect neurons Hidden-Out
\begin{comment}

\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden_Relu-\i) -- (Output-\j);
    }
}
\end{comment}
\draw[->, shorten >=1pt] (Hidden_Relu-1) -- node[above]{2}(Output-1);
\draw[->, shorten >=1pt] (Hidden_Relu-2) -- node[below]{-2}(Output-2);
\draw[->, shorten >=1pt] (Hidden_Relu-2) -- node[above]{-1}(Output-1);
\draw[->, shorten >=1pt] (Hidden_Relu-1) -- node[below]{-1}(Output-2);
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Input-\i) -- ++(-1,0)
        node[left]{$x_{\i}$};
}
 
% Outputs
\foreach \i in {1,...,\outputnum}
{            
    \draw[->, shorten <=1pt] (Output-\i) -- ++(1,0)
        node[right]{Output \#\i};
}
 
\end{tikzpicture}

\end{center}
 \caption{Attempt 2}
\end{figure}

==> sections/NN_manual_2.tex <==
    
% Input layer neurons'number
\newcommand{\inputnum}{2} 
 
% Hidden layer neurons'number
\newcommand{\hiddennum}{2}  

% Output layer neurons'number
\newcommand{\outputnum}{2} 

\begin{figure}[ht!]
\begin{center}
\begin{tikzpicture}
 
% Input Layer

    \node[circle,
     %node[align=center] 
     %text centered,
 label={[align=left]\normalsize \bf Input\\ \normalsize \textbf{Layer}\\~}, 
     %label=above:{\normalsize \bf Input Layer},
        %minimum size = 7mm,
        text width=4mm,
        text height=3mm,
        fill=orange!30] (Input-1) at (0,-1*1.7) {$x_1^{\textcolor{orange!30}{[1]}}$};

    \node[circle, 
        %minimum size = 7mm,
        text width=4mm,text height=3mm,
        fill=orange!30] (Input-2) at (0,-2*1.7) {$x_2^{\textcolor{orange!30}{[1]}}$};

% Hidden Layer

    \node[circle, 
        label={[align=left]\normalsize \bf Hidden\\ \normalsize \textbf{Layer}\\~}, 
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-1) at (2,-1*1.7) {$z_1^{[1]}$};
 \node[circle, 
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-2) at (2,-2*1.7) {$z_2^{[1]}$};
 
 \foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        %minimum size = 9mm,
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden_Relu-\i) at (4,-\i*1.7) {$h_{\i}^{\textcolor{blue!50}{[1]}}$};
}
% Output Layer
  

\node[circle, 
    label={[align=left]\normalsize \bf Output\\ \normalsize \textbf{Layer}\\~}, 
        %minimum size = 8mm,
    text width=4mm,text height=3mm,
    fill=purple!50,
    yshift=(\outputnum-\inputnum)*5 mm] (Output-1) at (6,-1*1.7) %{$\textcolor{purple!20}{h_1}^{[1]}$};
    {$y_1^{[1]}$};
    
    \node[circle, 
        %minimum size = 8mm,
        text width=4mm,text height=3mm,
        fill=purple!50,
        yshift=(\outputnum-\inputnum)*5 mm
    ] (Output-2) at (6,-2*1.7){$y_2^{[1]}$};

 
% Connect neurons In-Hidden
\begin{comment}
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Input-\i) -- (Hidden-\j);   
    }
}
\end{comment}
 \draw[->, shorten >=1pt] (Input-1) -- node[above] {$-2$}(Hidden-1);
 \draw[->, shorten >=1pt] (Input-2) --  node[below]{$2$}(Hidden-2);
 \draw[->, shorten >=1pt] (Input-1) --  node[above]{$1$}(Hidden-2);
  \draw[->, shorten >=1pt] (Input-2) --  node[below]{$1$}(Hidden-1);

% Connect neurons Hidden-Out
\foreach \i in {1,...,\hiddennum}
{
    %\foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt]  (Hidden-\i) -- node[above,sloped] {
        \small \text{ReLU}}(Hidden_Relu-\i);
    }
}
 

% Connect neurons Hidden-Out
\begin{comment}

\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden_Relu-\i) -- (Output-\j);
    }
}
\end{comment}
\draw[->, shorten >=1pt] (Hidden_Relu-1) -- node[above]{2}(Output-1);
\draw[->, shorten >=1pt] (Hidden_Relu-2) -- node[below]{-2}(Output-2);
\draw[->, shorten >=1pt] (Hidden_Relu-2) -- node[above]{-1}(Output-1);
\draw[->, shorten >=1pt] (Hidden_Relu-1) -- node[below]{-1}(Output-2);
% Inputs
\foreach \i in {1,...,\inputnum}
{            
    \draw[<-, shorten <=1pt] (Input-\i) -- ++(-1,0)
        node[left]{Input \#\i};
}
 %{$x_{\i}$}
% Outputs
\foreach \i in {1,...,\outputnum}
{            
    \draw[->, shorten <=1pt] (Output-\i) -- ++(1,0)
        node[right]{Output \#\i};
}
\end{tikzpicture}
\caption{Attempt 3}
\end{center}

\end{figure}
 

==> sections/NN_manual_4.tex <==
    
% Input layer neurons'number
\renewcommand{\inputnum}{2} 
 
% Hidden layer neurons'number
\renewcommand{\hiddennum}{2}  

% Output layer neurons'number
\renewcommand{\outputnum}{2} 
 
 \begin{figure}[ht!]
 \begin{center}

\begin{tikzpicture}
 
% Input Layer

    \node[circle,
     %node[align=center] 
     %text centered,
 label={[align=left]\normalsize \bf Input\\ \normalsize \textbf{Layer}\\~}, 
     %label=above:{\normalsize \bf Input Layer},
        %minimum size = 7mm,
        text width=4mm,
        text height=3mm,
        fill=orange!30] (Input-1) at (0,-1*1.7) {$x_1^{\textcolor{orange!30}{[1]}}$};

    \node[circle, 
        %minimum size = 7mm,
        text width=4mm,text height=3mm,
        fill=orange!30] (Input-2) at (0,-2*1.7) {$x_2^{\textcolor{orange!30}{[1]}}$};

% Hidden Layer

    \node[circle, 
        label={[align=left]\normalsize \bf Hidden\\ \normalsize \textbf{Layer}\\~}, 
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-1) at (2,-1*1.7) {$z_1^{[1]}$};
 \node[circle, 
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden-2) at (2,-2*1.7) {$z_2^{[1]}$};
 
 \foreach \i in {1,...,\hiddennum}
{
    \node[circle, 
        %minimum size = 9mm,
        text width=4mm,text height=3mm,
        fill=blue!50,
        yshift=(\hiddennum-\inputnum)*5 mm
    ] (Hidden_Relu-\i) at (4,-\i*1.7) {$h_{\i}^{\textcolor{blue!50}{[1]}}$};
}
% Output Layer
  

\node[circle, 
    label={[align=left]\normalsize \bf Output\\ \normalsize \textbf{Layer}\\~}, 
        %minimum size = 8mm,
    text width=4mm,text height=3mm,
    fill=purple!50,
    yshift=(\outputnum-\inputnum)*5 mm] (Output-1) at (6,-1*1.7) %{$\textcolor{purple!20}{h_1}^{[1]}$};
    {$y_1^{[1]}$};
    
    \node[circle, 
        %minimum size = 8mm,
        text width=4mm,text height=3mm,
        fill=purple!50,
        yshift=(\outputnum-\inputnum)*5 mm
    ] (Output-2) at (6,-2*1.7){$y_2^{[1]}$};

 
% Connect neurons In-Hidden
\begin{comment}
\foreach \i in {1,...,\inputnum}
{
    \foreach \j in {1,...,\hiddennum}
    {
        \draw[->, shorten >=1pt] (Input-\i) -- (Hidden-\j);   
    }
}
\end{comment}
 \draw[->, shorten >=1pt] (Input-1) -- node[above] {$-2$}(Hidden-1);
 \draw[->, shorten >=1pt] (Input-2) --  node[below]{$2$}(Hidden-2);
 \draw[->, shorten >=1pt] (Input-1) --  node[above]{$1$}(Hidden-2);
  \draw[->, shorten >=1pt] (Input-2) --  node[below]{$1$}(Hidden-1);

% Connect neurons Hidden-Out
\foreach \i in {1,...,\hiddennum}
{
    %\foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt]  (Hidden-\i) -- node[above,sloped] {\em \small ReLU}(Hidden_Relu-\i);
    }
}
 

% Connect neurons Hidden-Out
\begin{comment}

\foreach \i in {1,...,\hiddennum}
{
    \foreach \j in {1,...,\outputnum}
    {
        \draw[->, shorten >=1pt] (Hidden_Relu-\i) -- (Output-\j);
    }
}
\end{comment}
\draw[->, shorten >=1pt] (Hidden_Relu-1) -- node[above]{2}(Output-1);
\draw[->, shorten >=1pt] (Hidden_Relu-2) -- node[below]{-2}(Output-2);
\draw[->, shorten >=1pt] (Hidden_Relu-2) -- node[above]{-1}(Output-1);
\draw[->, shorten >=1pt] (Hidden_Relu-1) -- node[below]{-1}(Output-2);
% Inputs

 %{$x_{\i}$}
% Outputs

\end{tikzpicture}

\end{center}
\caption{Attempt 5}

\end{figure} 

==> sections/new_table.tex <==
\begin{table}[h]
%\begin{adjustbox}{center}
    \renewcommand{\arraystretch}{1.2} % For vertical spacing
\setlength{\tabcolsep}{0.5em} % For horizontal spacing
\begin{tabular}{@{}cccccccc@{}}
%\begin{tabular}{@{}lllllll@{}}
\toprule
%\multicolumn{1}{|p{2cm}|}{\centering \#  nodes per layer} & 
\textbf{\#nodes} & \textbf{\#SMT var.} & \textbf{Strict  Equiv.}& $\boldsymbol{L_{1}}$ \textbf{equiv.} & $\boldsymbol{L_{2}}$ \textbf{equiv.} & {\bf $L_{\infty}$ equiv.} & \textbf{Argmax equiv.} \\\midrule
%\multicolumn{1}{|p{2cm}|}{\centering \# SMT var.} &   
%\multicolumn{1}{|p{2cm}|}{\centering Strict \\ Equiv.} & 
%\multicolumn{1}{|p{2cm}|}{\centering $L_{1}$ equiv. } & \multicolumn{1}{|p{2cm}|}{\centering $L_{2}$ equiv.} & \multicolumn{1}{|p{2cm}|}{\centering $L_{\infty}$ equiv.} & \multicolumn{1}{|p{2cm}|}{\centering Argmax \\ Equiv.} \\ \midrule
5 & 378 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04  \\ 
10 & 938 & 0.1 & 0.09 & 0.09 & 0.09 & 0.1  \\ 
15 & 1698 & 0.15 & 0.15 & 0.16 & 0.16 & 0.15 \\ 
20 & 2658 & 0.24 & 0.24 & 0.24 & 0.23 & 0.23  \\ 
30 & 5178 & 0.4 & 0.39 & 0.4 & 0.39 & 0.42  \\ 
40 & 8498 & 0.62 & 0.62 & 0.63 & 0.63 & 0.63  \\ 
50 & 12618 & 0.87 & 0.91 & 0.89 & 0.88 & 0.92  \\ 
60 & 17538 & 1.17 & 1.2 & 1.17 & 1.16 & 1.23  \\ 
\bottomrule
\end{tabular}
%\end{adjustbox}
\caption{Sanity Check on BitVec dataset - 2nd Architecture;\#nodes: number of nodes (neurons) per hidden layer, \#SMT var.: number of SMT variables}
%NK: add time [sec], number of SMT variabls, $\epsilon$, number of hidden layers
% always satsified 
\label{tab:Table 3}
\end{table}


==> sections/todo.tex <==
\newpage
\red{To DO from 9.3.2022 -- REMOVE BEFORE SUBMITTING TO WORKSHOP AND ARXIV}
\begin{enumerate}

    \item future TO DO
    \begin{itemize}
        \item Use MILP solver
        \item Understand, compare and analyze Saphire.\url{https://github.com/wenkokke/sapphire/blob/master/tutorial/tutorial-sapphire.ipynb}
        \item Find state-of-the-art tools for NN verification from VNN-Comp~\url{https://sites.google.com/view/vnn2021}
        \item Choose 1-2 of them (alpha-beta crown or ERAN), download and import our NNs. FInd one of our problems and reduce it to a reachability problem. Then compare with our reuslts. 
    \end{itemize}
\end{enumerate}
